Uniform approximation in classical weak convergence theory

A common statistical task lies in showing asymptotic normality of certain statistics. In many of these situations, classical textbook results on weak convergence theory suffice for the problem at hand. However, there are quite some scenarios where stronger results are needed in order to establish an asymptotic normal approximation uniformly over a family of probability measures. In this note we collect some results in this direction. We restrict ourselves to weak convergence in $\mathbb R^d$ with continuous limit measures.

==> supplement_intro.tex <==
%
%		\title{\bf Supplement to "Adaptive confidence sets for kink estimation"}
%	\author{  Viktor Bengs
%		and 
%		Hajo Holzmann\footnote{Corresponding author, Email: holzmann@mathematik.uni-marburg.de} 	\\
%		Department of Mathematics and Computer Science, Philipps-Universit\"at Marburg}
%	\maketitle
%	
%	
%\begin{abstract}
%	
%	%
%	This supplementary material contains detailed proofs of the results in \citet{be2018main} as well as a   procedure  on constructing appropriate kernels for the main paper and further simulation results. 
%%	
%	In addition, some results on weak convergence uniformly over families of probability measures, and also findings on sub-Gaussian processes from \citet{viens2007supremum} are collected.
%	%	
%	%		 
%\end{abstract}
%%

% 
		
		
		
		\begin{frontmatter}
			
			\title{Uniform weak convergence theory}
			\runtitle{Uniform weak convergence theory}
			
	\begin{aug}
	\author{\fnms{Viktor}  \snm{Bengs}\thanksref{t1}\ead[label=e1]{bengs@mathematik.uni-marburg.de}}
	\and
	\author{\fnms{Hajo} \snm{Holzmann}\thanksref{t1,t2}\ead[label=e2]{holzmann@mathematik.uni-marburg.de}}
	%			\ead[label=u1,url]{http://www.foo.com}
	
	
	
	\address{Department of Mathematics and Computer Science. \\ Philipps-Universit\"at Marburg.	\\Hans-Meerwein-Stra\ss e, 35032 Marburg, Germany   \\
		\printead{e1,e2}}
	
	\thankstext{t1}{Supported by DFG Grant Ho 3260/5-1.}
	\thankstext{t2}{Corresponding author.}
	\runauthor{V. Bengs and H. Holzmann}
	
	\affiliation{ Philipps-Universit\"at Marburg.}
	
\end{aug}
			
			\begin{abstract} \
%				
				This paper provides some useful results on weak convergence uniformly over families of probability measures.
%				\\
				Although not new ... for the sake of easy access.
				%
				%		 	 
			\end{abstract}
			
			\begin{keyword}
				\kwd{Continuous mapping theorem}
				\kwd{Convergence in distribution}
				\kwd{Cram\'er-Wold theorem}
				\kwd{L\'evy's continuity theorem}
				\kwd{Lindeberg-Feller theorem}
				\kwd{Slutzky's theorem}
			\end{keyword}
			
		\end{frontmatter}
		
		
